Combining Deep Learning and Model-Based Methods for Robust Real-Time Semantic Landmark Detection

Compared to abstract features, significant objects, so-called landmarks, are a more natural means for vehicle localization and navigation, especially in challenging unstructured environments. The major challenge is to recognize landmarks in various lighting conditions and changing environment (growing vegetation) while only having few training samples available. We propose a new method which leverages Deep Learning as well as model-based methods to overcome the need of a large data set. Using RGB images and light detection and ranging (LiDAR) point clouds, our approach combines state-of-the-art classification results of Convolutional Neural Networks (CNN), with robust model-based methods by taking prior knowledge of previous time steps into account. Evaluations on a challenging real-wold scenario, with trees and bushes as landmarks, show promising results over pure learning-based state-of-the-art 3D detectors, while being significant faster.

==> ddcrp.tex <==
\begin{tikzpicture}%[scale=0.8, transform shape]
\tikzstyle{table}=[shape=circle,draw=blue!50,fill=blue!10,minimum size=1.5cm]
\tikzstyle{customer}=[shape=rectangle,draw=green!60!white,fill=green!10!white]
\tikzstyle{emptybox}=[shape=rectangle,draw=white,fill=white]
\tikzstyle{whitebox}=[shape=rectangle,draw=white,fill=white]
\tikzstyle{bigbox} = [draw=blue!50, thick, fill=blue!5, rounded corners, rectangle]
\tikzset{
	main/.style={circle,minimum size=2cm, thick, draw =black!80, node distance = 8mm},
	connect/.style={-latex, thick},
	emptybox/.style={rectangle,minimum width =60pt, minimum height=40pt,fill=blue!5,node distance = 10mm},
	box/.style={rectangle, minimum width =60pt, minimum height=40pt,text width=5em,text centered, draw=gray!30!black,fill=gray!30!white,node distance = 10mm}
}

\node[table](T1){Table 1};
\node[table](T2)[right=2.5cm of T1]{Table 2};
%\node[table](T3)[right=2.5cm of T2]{Table 3};

\node[customer](c1)[left=0.5cm of T1]{$ C_1 $};
\node[customer](c2)[right=0.5cm of T1]{$ C_2 $};
\node[customer](c4)[below=0.5cm of T1]{$ C_4 $};
\node[customer](c3)[right=0.5cm of T2]{$ C_3 $};


\node[customer](c22)[above=2.cm of T1]{$ C_2 $};
\node[customer](c11)[left=0.5cm of c22]{$ C_1 $};
\node[customer](c33)[right=0.5cm of c22]{$ C_3 $};
\node[customer](c44)[right=0.5cm of c33]{$ C_4 $};

\draw [arrow] (c22) to (c11);
\draw [arrow,bend right=30] (c44.north) to (c11.north);
\draw [arrow,bend left=30] (c44.south) to (c22.south);
%\draw [arrow] (c11) to (c22);
\node[whitebox](empty)[above= 1.8cm of c2]{};
\node[whitebox](empty2)[above= 0.4cm of c2]{};
\draw[arrow,dotted] (empty) -- (empty2);

%\begin{pgfonlayer}{background}
%	\node[shape=rectangle,draw=red!50,thick,fill=red!10,rounded corners] [fit = (input) (instances)]{};
%\end{pgfonlayer}
%\begin{pgfonlayer}{background}
%	\node[bigbox] [fit = (proposals) (projection)] {};
%\end{pgfonlayer}
%\begin{pgfonlayer}{background}
%	\node[bigbox] [fit = (filter) (gdpf)] {};
%\end{pgfonlayer}
%\begin{pgfonlayer}{background}
%	\node[bigbox] [fit = (pclass) (pointnet)] {};
%\end{pgfonlayer}
\end{tikzpicture}

==> iou.tex <==
\tikzset{
	box1/.style={%
		draw=black, thick,
		rectangle,
	%	rounded corners,
	    minimum height=1.5cm,
		minimum width=1.5cm
	},
}
\tikzset{
	box2/.style={%
		draw=black, thick,
		rectangle,
	%	rounded corners,
		minimum height=0.75cm,
		minimum width=0.75cm
	},
}
% Set A and B
\begin{tikzpicture}
\node[box1, fill=red, fill opacity=0.1] (c2) at (0,0) {};
\node[box1, fill=blue, fill opacity=0.1] (c1) at (0.75,0.75) {};
\node[box2,fill=green] (c3) at (0.375,0.375 ){};

\draw (-1.31,-1.21) -- (2.,-1.21){};
\node[box1, fill=green] (c2) at (0,-3) {};
\node[box1, fill=green] (c1) at (0.75,-2.25) {};
\node at (-1.91,-1.21) {IoU $ = $};
\node at (-0.375,-0.5) {$ 3 $D};
\node at (1.15,1.25) {$ 2 $D};
\node at (-0.375,-3.5) {$ 3 $D};
\node at (1.15,-1.75) {$ 2 $D};

\end{tikzpicture}


==> preliminaries.tex <==
\section{Related Work} \label{sec:related_works}

\begin{figure}
	\include{data/pipeline}
	\caption{lore}
\end{figure}
\begin{figure}
	\include{data/modified_pointnet}
	\caption{lore lipsum}
\end{figure}
